Mixture of Inference Networks for VAE-based Audio-visual Speech Enhancement

In this paper, we are interested in unsupervised (unknown noise) audio-visual speech enhancement based on variational autoencoders (VAEs), where the probability distribution of clean speech spectra is simulated using an encoder-decoder architecture. The trained generative model (decoder) is then combined with a noise model at test time to estimate the clean speech. In the speech enhancement phase (test time), the initialization of the latent variables, which describe the generative process of clean speech via decoder, is crucial, as the overall inference problem is non-convex. This is usually done by using the output of the trained encoder where the noisy audio and clean visual data are given as input. Current audio-visual VAE models do not provide an effective initialization because the two modalities are tightly coupled (concatenated) in the associated architectures. To overcome this issue, inspired by mixture models, we introduce the mixture of inference networks variational autoencoder (MIN-VAE). Two encoder networks input, respectively, audio and visual data, and the posterior of the latent variables is modeled as a mixture of two Gaussian distributions output from each encoder network. The mixture variable is also latent, and therefore the inference of learning the optimal balance between the audio and visual inference networks is unsupervised as well. By training a shared decoder, the overall network learns to adaptively fuse the two modalities. Moreover, at test time, the visual encoder, which takes (clean) visual data, is used for initialization. A variational inference approach is derived to train the proposed generative model. Thanks to the novel inference procedure and the robust initialization, the proposed MIN-VAE exhibits superior performance on speech enhancement than using the standard audio-only as well as audio-visual counterparts.

==> coverletter-R3.tex <==
\begin{coverletter}{Mixture of Inference Networks for VAE-based Audio-visual Speech Enhancement}{T-SP-27172-2020}


\begin{answereditor}{As you can see, one reviewer still has some concerns about the experimental section. In particular, the baseline is low. The authors are encouraged to use more current benchmarking techniques, if possible.}

We would like to thank the Associate Editor and the Reviewer for their constructive comments and suggestions. We have carefully followed their recommendations and revised the paper accordingly. 

\textbf{An annotated version of the revised manuscript, in which the modifications, novel paragraphs and sections are highlighted in green and numbered R1, R2, 
etc., is attached with this cover letter. Our detailed answers below refer to these annotations, e.g. ``Revision\#1 on Page~2'' refers to annotation R1 on 
Page 2 of the attached revised manuscript}. 

\end{answereditor}

\begin{answerreviewer}[Recommendation: RQ - Review Again After Major Changes]

\qa{Thank the authors for their great effort. The manuscript was written clearly. Most of my questions were addressed.}
{We really appreciate your encouraging feedback.}

\qa{However, my major concern is the performance in the experiment section. The A-VAE baseline in Figs. 2 and 3 provides higher STOI scores when comparing with other AV methods. For MIN-VAE-v2, the average PESQ improvement from AV-VAE is about 0.1. These results suggest the visual features are not handling well by VAE and thus provides less advantage for the VAE-based AVSE system. Therefore, improving from low AV-VAE results might be easy with the applied fusion technique.}
{First of all, please note that the ultimate versions of the proposed algorithms are the ones presented in Fig.~4 (and not Fig.~3). These correspond to the case when some noise was added to the audio input of the MIN-VAE during training, so as to learn a better balance between the contributions of audio and visual modalities, as explained in the last paragraph of Section IV.B, right before~\refcm{noise}. The same strategy has also been tried with A-VAE and AV-VAE, by adding noise to their audio-encoders' inputs. However, no performance improvements were observed. We have added an explanation to the paper. Please refer to \refcm{noise}. 
	
To have a fair performance comparison among different VAE architectures for speech enhancement, we should pay attention to some points. First, as a well-established observation, visual modality is most helpful when the input audio noise is high (low SNR regimes). This means that audio-visual speech enhancement is expected to outperform audio-only counterpart mainly in high levels of audio noise. Keeping that in mind, we see from Fig.~4 that the proposed MIN-VAE-v2 consistently outperform A-VAE at low SNR levels, and it demonstrates a much better performance than the AV-VAE baseline. Regarding the improvement margin, we see that on average, MIN-VAE-v2 outperforms AV-VAE, about 1dB in terms of SDR (high SNRs), more than 0.1 in terms of PESQ, and about 0.03-0.04 in terms of STOI. Overall, even if different MIN-VAE strategies may obtain the best improvement over AV-VAE depending on the measure and on the SNR, the superiority of MIN-VAE w.r.t.\ the AV-VAE is clear, since MIN-VAE is able to adapt its fusion strategy at each frame, while AV-VAE is systematically fusing the auditory and visual modalities. We agree that these values are not very significant, but they well-demonstrate the role of visual modality in speech enhancement, and the importance of latent initialization and audio-visual fusion, as the main contributions of the current paper. Moreover, in our previous work [26], the (unsupervised) AV-VAE speech enhancement has been experimentally shown to outperform a supervised deep neural network-based method presented in [25] (\refcm{comparison}). To make these points clearer, we have added some explanations to Section IV.B. Please refer to \refcm{experiments}.

It should also be noted that we have experimented with very simple VAE architectures (both for audio-only and audio-visual settings) composed of fully-connected layers. More sophisticated VAE architectures, consisting of convolutional and recurrent layers, are expected to provide a better performance, especially because they take into account the temporal dynamics of audio and visual time frames [35]. Nevertheless, implementation of such architectures poses some challenges for the inference (speech enhancement) phase, and we are seriously working on that as a follow-up of our current work. Please refer to \refcm{future}.}


\end{answerreviewer}

\end{coverletter}

\twocolumn
\setcounter{page}{1}
\setcounter{figure}{0}

